A Lipschitz Bandits Approach for Continuous Hyperparameter Optimization

One of the most critical problems in machine learning is HyperParameter Optimization (HPO), since choice of hyperparameters has a significant impact on final model performance. Although there are many HPO algorithms, they either have no theoretical guarantees or require strong assumptions. To this end, we introduce BLiE -- a Lipschitz-bandit-based algorithm for HPO that only assumes Lipschitz continuity of the objective function. BLiE exploits the landscape of the objective function to adaptively search over the hyperparameter space. Theoretically, we show that $(i)$ BLiE finds an $\epsilon$-optimal hyperparameter with $\mathcal{O} \left( \epsilon^{-(d_z + \beta)}\right)$ total budgets, where $d_z$ and $\beta$ are problem intrinsic; $(ii)$ BLiE is highly parallelizable. Empirically, we demonstrate that BLiE outperforms the state-of-the-art HPO algorithms on benchmark tasks. We also apply BLiE to search for noise schedule of diffusion models. Comparison with the default schedule shows that BLiE schedule greatly improves the sampling speed.

==> tex/intro.tex <==
\section{Introduction}

% Hyperparameter 

A Multi-Armed Bandit (MAB) algorithm seeks to balance off the tension between exploring the decision space and exploiting the good options. Roughly speaking, these algorithms try to make few mistakes while searching for the optimal decision. Due to this characteristic, MAB algorithms are often used in environments where trying an action is not cheap \citep[e.g.,][]{}. When exploitation is not as important as exploration, the MAB problem becomes the \emph{pure exploration problem} or the Best Arm Identification (BAI) problem, where the task 
is finding the best arm efficiently. MAB and BAI problems have attracted tremendous amount of attention in recent years. Among the uncountably many variations of the classic MAB model \citep{}, bandit learning with \emph{batched feedback} forms an important line of works \citep{}. In bandit problems with batched feedback, the learning agent does not immediately observe reward after pulling arms. Instead, they collect the reward observations every several arm pulls. Effectively, the batched feedback setting allows the learning agent to ``parallelize'' arm pulling: They can pull several arms in parallel, and collect the rewards all together. The authors recommend \citep{} for general exposition on MAB problems. 

% While it is hopeless to 


HyperParameter Optimization (HPO) problems become increasingly important in recent years, urged by increasing size of deep learning models \citep[e.g.,][]{}. HPO problems often carry structures that are not common in bandit problems. For example, in HPO usually a budget is associated to training a hyperparameter configuration. This budget models training resource consumption (e.g., number of training iterations etc). Usually allocating more budget to one hyperparameter means that more accurate learning output are observed \citep{}. Such structures make HPO problems theoretically intriguing and practically important. HPO problems naturally use many bandit learning principles. Since tuning hyperparameters are often not cheap, bandit learning principles can aid HPO tasks by minimizing number of trials. When applying bandit learning principles to HPO, one models the hyperparameter configurations as arms, and the learning output (e.g, testing accuracy/validation accuracy) as rewards. With this correspondence, the HPO task can be modeled as a bandit learning process: One selects some hyperparameter configurations to train models, collect learning output of these hyperparameter configurations, and repeat this procedure until the total training budget runs out. 

% -------------------------------------------------

Lipschitzness indeed models the behavior of many hyperparameters, of which the learning rate is an important example. Practitioners often find learning rate to be one of the most important hyperparameter to training a good model. Since the learning output does not always increase/decrease with learning rate, parameters like learning rate may not be simply modeled by a linear or polynomial model. For such hyperparameters, Lipschitz bandit models are natural choice. \textcolor{red}{(name a few other examples, e.g., some hyperparameters for Adam, etc. )} 

The batched feedback setting also comes in handy for HPO problems. For HPO problems, it is desirable to train several different hyperparameter configurations in parallel. In standard bandit learning settings, the agent usually needs to observe the reward immediately after arm pulling, so that subsequent decisions can be made. In batched feedback setting, one only needs to collect rewards every several arm pulls. Effectively, algorithms for the batched feedback setting allows one to train several hyperparameter configurations in parallel. Compared to the standard sequential decision making setting, this batched feedback setting can significantly improve HPO efficiency. 


In this paper, we study pure exploration for Lipschitz bandits with batched feedback, and apply such algorithms to HPO problems. We investigate the \emph{Batched Lipschitz Narrowing} (BLiN) algorithm \citep{} in a setting with training budget constraints, and study its behavior for pure exploration tasks. The BLiN algorithm collects rewards every several arm pulls, and adaptively eliminates regions of low rewards. \textcolor{red}{(describe the algorithm with budget constraints)}. 

Performance of the BLiN algorithm for pure exploration tasks is measured by \emph{simple regret}. Simple regret is the gap between the optimal arm and the best arm output by BLiN (within a fixed total budget). The \emph{simple regret} of the BLiN algorithm is controlled by a quantity describing the landscape of the learning output function, called \emph{zooming dimension} \citep{}. Lower zooming dimension means smaller simple regret and thus faster identification of good hyperparameter configurations. For HPO tasks, higher correlation in the hyperparameters implies lower zooming dimension. Usually, the hyperparameters are highly correlated, and thus BLiN naturally efficiently identify good hyperparameter configurations. In fact, we have observed that BLiN can automatically find patterns in hyperparameter configurations. \textcolor{red}{(briefly describe the main theorems, new findings on hyperparameter choice, and summarize the empirical observations)} 


The rest of the paper is organized as follows \textcolor{red}{......}




